To Combine or Not? Consolidating Horizontal Acquisitions in Multi-sided Market

When a parent company acquires a horizontal competitor on the same side of a multi-sided market, it must decide whether to fully integrate the acquired platform or keep it as a separate brand. We study this in the context of Uber's acquisition of Postmates, using novel consumer receipt data that tracks food delivery spending. Employing an Age-Period-Cohort (APC) decomposition, we isolate the merger's effect on consumer spending while controlling for lifecycle and cohort effects. We find that Postmates users sharply reduced their spending on the platform after the merger, but spending shifted not only to UberEats, but also to competitors like DoorDash and Grubhub. Consumers who used multiple platforms and had low pre-merger activity on Postmates were more 'sticky', showing little change. Comparing our APC results with a standard Difference-in-Differences (DiD) design, we find the DiD underestimates the merger's total impact by missing market-wide effects. Our findings suggest that in multi-sided markets, keeping acquired platforms separate can be beneficial; dissolving them may push demand to competitors, and some sticky multihoming users may not shift spending at all.

==> table1.tex <==

\begin{table}
\centering
\begin{tblr}[         %% tabularray outer open
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]},
column{2}={}{halign=c,},
column{1}={}{halign=l,},
hline{8}={1,2}{solid, black, 0.05em},
}                     %% tabularray inner close
\toprule
Budget Share for primary platform & (1) \\ \midrule %% TinyTableHeader
Treatment X Post & \num{0.124} \\
& (\num{0.014}) \\
Total covid cases & \num{-0.000} \\
& (\num{0.000}) \\
Work place close order & \num{0.006} \\
& (\num{0.023}) \\
Num.Obs. & \num{10112} \\
FE: user\_id\_factor & X \\
FE: year\_month\_factor & X \\
Standard errors clustered at app level & X \\
\bottomrule
\end{tblr}
\end{table}

==> tabs/APC_robust_table1_AR_sensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{Robustness: Sensitivity to AR Search Range}
\label{tab:robust_ar}
\begin{tabular}{lccccc}
\toprule
Search Range & Selected & AIC & Shift (pp) & 95\% CI Lo & 95\% CI Hi \\
\midrule
AR(0-3) & AR(2) & 111.1 & -19.727 & -31.133 & -8.322 \\
AR(0-6) & AR(6) & 107.7 & -19.802 & -29.806 & -9.797 \\
AR(0-9) & AR(6) & 107.7 & -19.802 & -29.806 & -9.797 \\
\bottomrule
\multicolumn{6}{l}{\footnotesize O\&M approach. Detrended with linear trend + bs(month, 3). Full controls.} \\
\end{tabular}
\end{table}


==> tabs/APC_robust_table2_knot_sensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{Robustness: Sensitivity to Seasonality Detrending (B-Spline Knots)}
\label{tab:robust_knots}
\begin{tabular}{lccccc}
\toprule
Knots & Selected AR & AIC & Shift (pp) & 95\% CI Lo & 95\% CI Hi \\
\midrule
3 & AR(6) & 107.7 & -19.802 & -29.806 & -9.797 \\
4 & AR(6) & 100.8 & -21.496 & -30.770 & -12.222 \\
5 & AR(6) & 101.7 & -21.207 & -30.595 & -11.820 \\
6 & AR(6) & 102.1 & -22.313 & -30.757 & -13.869 \\
\bottomrule
\multicolumn{6}{l}{\footnotesize O\&M approach. AR search 0--6. Full controls.} \\
\end{tabular}
\end{table}


==> tabs/APC_robust_table3_controls_spec.tex <==
\begin{table}[htbp]
\centering
\caption{Robustness: O\&M Post-Merger Shift Across Control Sets}
\label{tab:robust_controls}
\begin{tabular}{lccccc}
\toprule
Specification & AR(p) & Shift (pp) & 95\% CI Lo & 95\% CI Hi \\
\midrule
1: No controls & AR(4) & -25.725 & -30.070 & -21.379 \\
2: + User (sync/multi) & AR(4) & -29.952 & -34.706 & -25.199 \\
3: + COVID & AR(4) & -29.087 & -39.198 & -18.976 \\
4: + Restaurants (full) & AR(6) & -19.802 & -29.806 & -9.797 \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Controls added cumulatively. bs(month, 3). AR search 0--6.} \\
\end{tabular}
\end{table}


==> tabs/APC_robust_table4_VAR_vs_AR.tex <==
\begin{table}[htbp]
\centering
\caption{Robustness: VAR vs AR Counterfactual — Post-Merger Shift}
\label{tab:robust_var}
\begin{tabular}{lcccc}
\toprule
Model & Shift (pp) & 95\% CI Lo & 95\% CI Hi & Granger $p$ \\
\midrule
AR(6) & -19.802 & -29.806 & -9.797 & --- \\
VAR(4) + COVID & -2643.293 & -3095.993 & -2190.593 & 0.5352 \\
\bottomrule
\multicolumn{5}{l}{\footnotesize VAR includes COVID cases (std) as second endogenous variable.} \\
\multicolumn{5}{l}{\footnotesize Granger $p$: test of COVID $\rightarrow$ period FE. Full controls in APC stage.} \\
\end{tabular}
\end{table}


==> tabs/APC_robust_table5_ACF_PACF.tex <==
\begin{table}[htbp]
\centering
\caption{ACF and PACF of Pre-Merger Detrended Period FE Residuals}
\label{tab:robust_acf}
\begin{tabular}{ccccc}
\toprule
Lag & ACF & Significant? & PACF & Significant? \\
\midrule
1 & -0.007 &  & -0.007 &  \\
2 & -0.509 & Yes & -0.509 & Yes \\
3 & -0.098 &  & -0.145 &  \\
4 & -0.150 &  & -0.579 & Yes \\
5 & 0.166 &  & -0.086 &  \\
6 & 0.197 &  & -0.458 &  \\
7 & 0.008 &  & -0.027 &  \\
8 & -0.020 &  & -0.366 &  \\
9 & -0.110 &  & 0.021 &  \\
10 & -0.038 &  & -0.285 &  \\
11 & 0.028 &  & 0.081 &  \\
12 & 0.031 &  & -0.227 &  \\
\midrule
\multicolumn{5}{l}{Ljung-Box Q(12) = 3.18, $p$ = 0.9942} \\
\bottomrule
\multicolumn{5}{l}{\footnotesize 95\% CI = $\pm$ 0.475. n = 17 pre-merger months.} \\
\end{tabular}
\end{table}


==> tabs/APC_table1_BP_break_tests.tex <==

\begin{table}[htbp]
\begin{center}
\begin{tabular}{l D{.}{.}{3.5} D{.}{.}{2.3} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5}}
\toprule
 & \multicolumn{1}{c}{All Users} & \multicolumn{1}{c}{Low PM Share} & \multicolumn{1}{c}{High PM Share} & \multicolumn{1}{c}{Single-Home} & \multicolumn{1}{c}{Multi-Home} & \multicolumn{1}{c}{High UE MSA} & \multicolumn{1}{c}{High PM MSA} & \multicolumn{1}{c}{Low UE MSA} & \multicolumn{1}{c}{High UE + Single} & \multicolumn{1}{c}{High UE + Multi} & \multicolumn{1}{c}{High Share + Single} & \multicolumn{1}{c}{High Share + Multi} \\
\midrule
Intercept   & 0.00         & 0.00   & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         \\
            & (1.82)       & (1.12) & (2.54)       & (1.80)       & (1.20)       & (1.90)       & (2.43)       & (1.75)       & (3.08)       & (1.42)       & (1.79)       & (2.24)       \\
Post-Merger & -27.63^{***} & -0.36  & -50.25^{***} & -42.54^{***} & -16.94^{***} & -21.10^{***} & -34.71^{***} & -27.66^{***} & -41.92^{***} & -12.44^{***} & -43.50^{***} & -31.88^{***} \\
            & (2.61)       & (1.61) & (3.65)       & (2.58)       & (1.73)       & (2.73)       & (3.48)       & (2.51)       & (4.42)       & (2.04)       & (2.56)       & (3.21)       \\
\midrule
R$^2$       & 0.77         & 0.00   & 0.85         & 0.89         & 0.74         & 0.64         & 0.75         & 0.79         & 0.73         & 0.53         & 0.90         & 0.75         \\
Adj. R$^2$  & 0.77         & -0.03  & 0.85         & 0.89         & 0.74         & 0.63         & 0.74         & 0.78         & 0.72         & 0.52         & 0.89         & 0.74         \\
Num. obs.   & 35           & 35     & 35           & 35           & 35           & 35           & 35           & 35           & 35           & 35           & 35           & 35           \\
\bottomrule
\multicolumn{13}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\caption{B\&P: Level Shift in Detrended Period FEs at Merger (Dec 2020)}
\label{tab:bp_break_tests}
\end{center}
\end{table}



==> tabs/APC_table2_OM_shifts.tex <==
\begin{table}[htbp]
\centering
\caption{O\&M: Avg Post-Merger Shift by Subgroup (ARIMA Counterfactual)}
\label{tab:om_shifts}
\begin{tabular}{llr}
\toprule
Subgroup & DV & Shift (pp) \\
\midrule
All Users & \% Postmates & -19.79 \\
All Users & \% UberEats & +7.27 \\
All Users & \% DoorDash & +15.93 \\
All Users & \% GrubHub & -5.01 \\
All Users & Orders & -0.07 \\
All Users & Spend & -0.37 \\
Low PM Share (<25%) & \% Postmates & +3.51 \\
High PM Share (>70%) & \% Postmates & -57.18 \\
Single-Homing & \% Postmates & -60.10 \\
Multi-Homing & \% Postmates & -20.93 \\
High Share + Single & \% Postmates & -60.10 \\
High Share + Multi & \% Postmates & -53.01 \\
High UE MSA & \% Postmates & -22.30 \\
High PM MSA & \% Postmates & -24.60 \\
Low UE MSA & \% Postmates & -32.06 \\
High UE + Single & \% Postmates & -57.54 \\
High UE + Multi & \% Postmates & -11.37 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/APC_table3_BP_all_DVs.tex <==

\begin{table}[htbp]
\begin{center}
\begin{tabular}{l D{.}{.}{3.5} D{.}{.}{2.5} D{.}{.}{2.5} D{.}{.}{2.5} D{.}{.}{2.3} D{.}{.}{2.3}}
\toprule
 & \multicolumn{1}{c}{\% Postmates} & \multicolumn{1}{c}{\% UberEats} & \multicolumn{1}{c}{\% DoorDash} & \multicolumn{1}{c}{\% GrubHub} & \multicolumn{1}{c}{Orders} & \multicolumn{1}{c}{Spend} \\
\midrule
Intercept   & 0.00         & -0.00       & -0.00      & -0.00      & 0.00   & -0.00  \\
            & (1.82)       & (1.27)      & (0.88)     & (0.31)     & (0.10) & (3.66) \\
Post-Merger & -27.63^{***} & 16.73^{***} & 9.60^{***} & 1.63^{***} & -0.17  & -4.58  \\
            & (2.61)       & (1.82)      & (1.26)     & (0.45)     & (0.14) & (5.26) \\
\midrule
R$^2$       & 0.77         & 0.72        & 0.64       & 0.29       & 0.04   & 0.02   \\
Adj. R$^2$  & 0.77         & 0.71        & 0.63       & 0.27       & 0.01   & -0.01  \\
Num. obs.   & 35           & 35          & 35         & 35         & 35     & 35     \\
\bottomrule
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\caption{B\&P: Post-Merger Level Shift in Detrended Period FEs by DV}
\label{tab:bp_break_dvs}
\end{center}
\end{table}



==> tabs/APC_table4_het_summary.tex <==
\begin{table}[htbp]
\centering
\caption{Heterogeneous Post-Merger Effects on \% Postmates Spending}
\label{tab:het_summary}
\begin{tabular}{lrr}
\toprule
Subgroup & B\&P Shift (pp) & O\&M Shift (pp) \\
\midrule
Low PM Share (<25%) & -0.36 & +3.51 \\
High PM Share (>70%) & -50.25 & -57.18 \\
Single-Homing & -42.54 & -60.10 \\
Multi-Homing & -16.94 & -20.93 \\
High + Single & -43.50 & -60.10 \\
High + Multi & -31.88 & -53.01 \\
High UE MSA & -21.10 & -22.30 \\
High PM MSA & -34.71 & -24.60 \\
Low UE MSA & -27.66 & -32.06 \\
High UE + Single & -41.92 & -57.54 \\
High UE + Multi & -12.44 & -11.37 \\
\bottomrule
\end{tabular}
\vspace{0.3em}
\parbox{\linewidth}{\footnotesize \textit{Notes:} B\&P: avg detrended period FE shift (post minus pre-merger). O\&M: avg gap between actual and ARIMA counterfactual period FEs.}
\end{table}


==> tabs/APC_table5_spec_curve_controls.tex <==
\begin{table}[htbp]
\centering
\caption{B\&P Specification Curve: Post-Merger Break in Period FEs Across Control Sets}
\label{tab:bp_spec_curve}
\begin{tabular}{lcccc}
\hline\hline
Specification & Break (pp) & SE & p-value & 95\% CI \\
\hline
1: No controls & -26.999 & (2.736) & 0.0000 & [-32.361, -21.636] \\
2: + User (sync, multi) & NA & (NA) & NA & [NA, NA] \\
3: + COVID & -27.631 & (2.609) & 0.0000 & [-32.745, -22.517] \\
4: + Restaurants (full) & -27.631 & (2.609) & 0.0000 & [-32.745, -22.517] \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Controls added cumulatively. User $\times$ time: issyncing, multi-homing indicators.} \\
\multicolumn{5}{l}{\footnotesize COVID: standardized cases (+ squared), workplace closures, gathering restrictions, stay-at-home.} \\
\multicolumn{5}{l}{\footnotesize Restaurant supply: new/common restaurants on Postmates and other platforms.} \\
\end{tabular}
\end{table}


==> tabs/APC_table6_OM_spec_curve_controls.tex <==
\begin{table}[htbp]
\centering
\caption{O\&M Specification Curve: Post-Merger Shift in Period FEs Across Control Sets}
\label{tab:om_spec_curve}
\begin{tabular}{lc}
\hline\hline
Specification & Shift (pp) \\
\hline
1: No controls & -25.660 \\
2: + User (sync, multi) & -29.847 \\
3: + COVID & -28.962 \\
4: + Restaurants (full) & -19.677 \\
\hline\hline
\multicolumn{2}{l}{\footnotesize Shift = mean post-merger detrended FE $-$ mean pre-merger detrended FE.} \\
\multicolumn{2}{l}{\footnotesize Controls aggregated to cohort $\times$ month level (mean within group).} \\
\end{tabular}
\end{table}


==> tabs/multihoming_descriptive.tex <==
\begin{tabular}{lcccc} \hline \hline
                    &Single-Homing&Multi-Homing\\
\hline
Median Number of Orders Per User&           2&          18\\
Average Number of Orders Per User&          12&          50\\
Average Amount Paid Per Order(\$)&       31.74&       33.59\\
Number of Active Users&       6,278&       3,816\\
Number of Total Orders&      74,343&     192,241\\
Total Revenue(\$)   &   2,359,547&   6,457,073\\
\hline
\hline \end{tabular}


==> tabs/multihoming_descriptive_postacq.tex <==
\begin{tabular}{lcccc} \hline \hline
                    &Single-Homing&Multi-Homing\\
\hline
Median Number of Orders Per User&           3&          18\\
Average Number of Orders Per User&          14&          42\\
Average Amount Paid Per Order(\$)&       33.12&       34.65\\
Number of Active Users&       4,160&       2,010\\
Number of Total Orders&      57,229&      84,570\\
Total Revenue(\$)   &   1,895,170&   2,930,587\\
\hline
\hline \end{tabular}


==> tabs/multihoming_descriptive_preacq.tex <==
\begin{tabular}{lcccc} \hline \hline
                    &Single-Homing&Multi-Homing\\
\hline
Median Number of Orders Per User&           2&          14\\
Average Number of Orders Per User&           9&          33\\
Average Amount Paid Per Order(\$)&       30.95&       32.51\\
Number of Active Users&       4,828&       2,527\\
Number of Total Orders&      42,118&      82,667\\
Total Revenue(\$)   &   1,303,457&   2,687,407\\
\hline
\hline \end{tabular}


==> tabs/summary_stats.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\hline\hline
                    &        Mean&          SD&         25q&      Median&         75q\\
\hline
total charged       &       33.16&       23.03&       19.21&       26.89&       40.33\\
service fee         &        2.75&        2.20&        1.30&        2.26&        3.60\\
delivery fee        &        1.59&        2.24&        0.00&        0.49&        2.99\\
\hline
Observations        &      269894&            &            &            &            \\
\hline\hline
\end{tabular}
}


==> tabs/table1_sample_construction.tex <==
\begin{table}[H]
\centering
\caption{Sample Construction}
\label{tab:sample_construction}
\begin{tabular}{clrrr}
\toprule
Step & Description & Users & Observations & MSAs \\
\midrule
0 & Raw data loaded & 10,094 & 266,542 & 699 \\
1 & Non-empty MSA & 10,073 & 265,910 & 626 \\
2 & Postmates users only (pre-merger) &  1,266 &  67,875 & 278 \\
3 & MSAs with >= 10 users &  1,144 &  58,931 &  47 \\
4 & Primary MSA only (most orders) &  1,144 &  55,228 &  47 \\
5 & Remove <5% PM budget share &    953 &  33,438 &  47 \\
6 & Remove >50% zero-PM months (post-adoption) &    798 &  25,664 &  47 \\
7 & Exclude Dec 2020 (merger month) &    798 &  24,833 &  47 \\
Final & Analysis panel (user × MSA × month) &    798 &   5,301 &  47 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/table2_summary_statistics.tex <==
\begin{table}[H]
\centering
\caption{Summary Statistics}
\label{tab:summary_stats_full}
\begin{tabular}{lrrrrrr}
\toprule
Variable & N & Mean & SD & Median & Min & Max \\
\midrule
\multicolumn{7}{l}{\textit{Panel A: User-Level Characteristics}} \\
Pre-merger PM spending share (%) & 766 & 71.73 & 32.63 & 91.21 & 5.04 & 100 \\
PM tenure (months before merger) & 766 & 10.58 & 5.63 & 9.99 & 0.99 & 18.04 \\
Avg monthly spending ($) & 798 & 94.21 & 127.26 & 51.16 & 1.57 & 1682.2 \\
Avg monthly orders & 798 & 2.84 & 3.33 & 1.67 & 1 & 32.04 \\
Avg % spending on Postmates & 798 & 63.2 & 35.07 & 66.67 & 0 & 100 \\
Months observed in panel & 798 & 6.64 & 7.49 & 3 & 1 & 34 \\
Is syncing (0/1) & 798 & 0.48 & 0.5 & 0 & 0 & 1 \\
Also uses UberEats (0/1) & 798 & 0.27 & 0.44 & 0 & 0 & 1 \\
Also uses DoorDash (0/1) & 798 & 0.36 & 0.48 & 0 & 0 & 1 \\
Also uses GrubHub (0/1) & 798 & 0.25 & 0.43 & 0 & 0 & 1 \\
\midrule
\multicolumn{7}{l}{\textit{Panel B: Monthly Panel Observations}} \\
% spending on Postmates & 5301 & 49.12 & 46.31 & 44.91 & 0 & 100 \\
% spending on UberEats & 5301 & 18.3 & 35.38 & 0 & 0 & 100 \\
% spending on DoorDash & 5301 & 23.01 & 39.01 & 0 & 0 & 100 \\
% spending on GrubHub & 5301 & 9.46 & 26.5 & 0 & 0 & 100 \\
Total monthly spending ($) & 5301 & 164.32 & 242.35 & 76.46 & 0 & 3148.02 \\
Total monthly orders & 5301 & 4.68 & 5.87 & 2 & 1 & 53 \\
COVID cases (standardized) & 5301 & 0.74 & 2.41 & -0.21 & -0.23 & 14.33 \\
Stay-at-home order (0/1) & 5301 & 0.15 & 0.32 & 0 & 0 & 1 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/table2a_summary_statistics.tex <==
\begin{table}[H]
\centering
\caption{Summary Statistics: User-Level Characteristics}
\label{tab:summary_stats}
\begin{tabular}{lrrrrrr}
\toprule
Variable & N & Mean & SD & Median & Min & Max \\
\midrule
Pre-merger PM spending share (%) & 766 & 71.73 & 32.63 & 91.21 & 5.04 & 100 \\
PM tenure (months before merger) & 766 & 10.58 & 5.63 & 9.99 & 0.99 & 18.04 \\
Avg monthly spending ($) & 798 & 94.21 & 127.26 & 51.16 & 1.57 & 1682.2 \\
Avg monthly orders & 798 & 2.84 & 3.33 & 1.67 & 1 & 32.04 \\
Avg % spending on Postmates & 798 & 63.2 & 35.07 & 66.67 & 0 & 100 \\
Months observed in panel & 798 & 6.64 & 7.49 & 3 & 1 & 34 \\
Is syncing (0/1) & 798 & 0.48 & 0.5 & 0 & 0 & 1 \\
Also uses UberEats (0/1) & 798 & 0.27 & 0.44 & 0 & 0 & 1 \\
Also uses DoorDash (0/1) & 798 & 0.36 & 0.48 & 0 & 0 & 1 \\
Also uses GrubHub (0/1) & 798 & 0.25 & 0.43 & 0 & 0 & 1 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/table2b_summary_statistics.tex <==
\begin{table}[H]
\centering
\caption{Summary Statistics: Monthly Panel}
\label{tab:summary_stats_panel}
\begin{tabular}{lrrrrrr}
\toprule
Variable & N & Mean & SD & Median & Min & Max \\
\midrule
% spending on Postmates & 5301 & 49.12 & 46.31 & 44.91 & 0 & 100 \\
% spending on UberEats & 5301 & 18.3 & 35.38 & 0 & 0 & 100 \\
% spending on DoorDash & 5301 & 23.01 & 39.01 & 0 & 0 & 100 \\
% spending on GrubHub & 5301 & 9.46 & 26.5 & 0 & 0 & 100 \\
Total monthly spending ($) & 5301 & 164.32 & 242.35 & 76.46 & 0 & 3148.02 \\
Total monthly orders & 5301 & 4.68 & 5.87 & 2 & 1 & 53 \\
COVID cases (standardized) & 5301 & 0.74 & 2.41 & -0.21 & -0.23 & 14.33 \\
Stay-at-home order (0/1) & 5301 & 0.15 & 0.32 & 0 & 0 & 1 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/table3_balance_table.tex <==
\begin{table}[H]
\centering
\caption{Pre-Merger Balance: Treatment vs.\ Control ($N_T$ = NA, $N_C$ = NA)}
\label{tab:balance}
\begin{tabular}{lrrrrrr}
\toprule
 & \multicolumn{2}{c}{Treated} & \multicolumn{2}{c}{Control} & & \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Variable & Mean & SD & Mean & SD & Difference & p-value \\
\midrule
Pre-merger PM share (%) & 70.901 & 33.238 & 73.171 & 31.554 & -2.27 & 0.3478 \\
PM tenure (months) & 10.822 & 5.596 & 10.158 & 5.666 & 0.664 & 0.1177 \\
Avg monthly spending ($) & 94.964 & 129.51 & 92.87 & 123.731 & 2.094 & 0.821 \\
Avg monthly orders & 2.898 & 3.39 & 2.721 & 3.23 & 0.177 & 0.465 \\
Avg % PM spending (all periods) & 63.86 & 35.224 & 62.226 & 34.777 & 1.634 & 0.5247 \\
Months observed & 6.837 & 7.831 & 6.29 & 6.862 & 0.547 & 0.3035 \\
Is syncing & 0.452 & 0.498 & 0.532 & 0.5 & -0.08** & 0.0295 \\
Also uses UberEats & 0.308 & 0.462 & 0.205 & 0.404 & 0.103*** & 0.0011 \\
Also uses DoorDash & 0.355 & 0.479 & 0.362 & 0.481 & -0.007 & 0.8514 \\
Also uses GrubHub & 0.238 & 0.426 & 0.263 & 0.441 & -0.025 & 0.4405 \\
Multi-platform user & 0.565 & 0.496 & 0.577 & 0.495 & -0.011 & 0.756 \\
\bottomrule
\multicolumn{7}{l}{\footnotesize \textit{Notes:} * $p<0.10$, ** $p<0.05$, *** $p<0.01$. Treatment: above-median pre-merger UberEats market share.} \\
\end{tabular}
\end{table}


==> tabs/table4_share_categories.tex <==
\begin{table}[H]
\centering
\caption{Spending Share Categories by Treatment Status}
\label{tab:share_categories}
\begin{tabular}{lrr}
\toprule
Postmates Share Category & Control & Treated \\
\midrule
High (>70%) & 169 (57.7\%) & 285 (56.5\%) \\
Low (<25%) & 36 (12.3\%) & 70 (13.9\%) \\
Medium (25-70%) & 74 (25.3\%) & 132 (26.2\%) \\
NA & 14 (4.8\%) & 17 (3.4\%) \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/table5_msa_summary.tex <==
\begin{table}[H]
\centering
\caption{MSA-Level Summary (Top 20 by User Count)}
\label{tab:msa_summary}
\begin{tabular}{llrrrrr}
\toprule
MSA & Group & UE Share (\%) & Users & Obs & Mean \% PM & Mean Spend. (\$) \\
\midrule
los angeles-long beach-anaheim, ca & Treated & 12.7 & 176 & 1380 & 60.54 & 205.64 \\
new york-newark-jersey city, ny-nj-pa & Control & 10.2 & 58 & 416 & 31.94 & 236.37 \\
miami-fort lauderdale-west palm beach, fl & Treated & 48.6 & 52 & 346 & 50.7 & 148.5 \\
phoenix-mesa-scottsdale, az & Control & 4 & 43 & 287 & 54.75 & 119.49 \\
atlanta-sandy springs-roswell, ga & Treated & 31.3 & 37 & 200 & 44.49 & 114.4 \\
san diego-carlsbad, ca & Control & 7.8 & 31 & 241 & 54.72 & 150.01 \\
san francisco-oakland-hayward, ca & Treated & 11.5 & 31 & 236 & 43.24 & 236.38 \\
portland-vancouver-hillsboro, or-wa & Treated & 13.5 & 23 & 215 & 51.12 & 123.29 \\
riverside-san bernardino-ontario, ca & Control & 6.3 & 22 & 120 & 55.46 & 130.53 \\
washington-arlington-alexandria, dc-va-md-wv & Treated & 11.5 & 22 & 138 & 46.9 & 176.56 \\
dallas-fort worth-arlington, tx & Treated & 31.8 & 20 & 149 & 34.99 & 255.36 \\
las vegas-henderson-paradise, nv & Control & 9.2 & 16 & 81 & 73.75 & 113.32 \\
nashville-davidson--murfreesboro--franklin, tn & Treated & 62.1 & 16 & 96 & 26.53 & 119.16 \\
charlotte-concord-gastonia, nc-sc & Treated & 16.8 & 15 & 117 & 59.43 & 131.49 \\
denver-aurora-lakewood, co & Control & 0.5 & 15 & 90 & 71.51 & 301.1 \\
orlando-kissimmee-sanford, fl & Treated & 22.9 & 15 & 99 & 34.91 & 124.67 \\
chicago-naperville-elgin, il-in-wi & Treated & 20 & 14 & 78 & 37.07 & 109.17 \\
sacramento--roseville--arden-arcade, ca & Control & 0.3 & 13 & 92 & 37.43 & 64.93 \\
boston-cambridge-newton, ma-nh & Treated & 29.2 & 12 & 54 & 31.6 & 116.83 \\
san jose-sunnyvale-santa clara, ca & Control & 4.6 & 12 & 75 & 19.72 & 163.29 \\
\bottomrule
\end{tabular}
\end{table}


==> tex/APC_robust_table4_VAR_vs_AR.tex <==
\begin{table}[htbp]
\centering
\caption{Robustness: VAR vs AR Counterfactual — Post-Merger Shift}
\label{tab:robust_var}
\begin{tabular}{lcccc}
\toprule
Model & Shift (pp) & 95\% CI Lo & 95\% CI Hi & Granger $p$ \\
\midrule
AR(4) & -40.333 & -53.072 & -27.594 & --- \\
VAR(4) + COVID & -47215.461 & -48302.832 & -46128.090 & 0.8548 \\
\bottomrule
\multicolumn{5}{l}{\footnotesize VAR includes COVID cases (std) as second endogenous variable.} \\
\multicolumn{5}{l}{\footnotesize Granger $p$: test of COVID $\rightarrow$ period FE. Full controls in APC stage.} \\
\end{tabular}
\end{table}


==> tex/APC_table1_BP_break_tests.tex <==

\begin{table}[htbp]
\begin{center}
\begin{tabular}{l D{.}{.}{3.5} D{.}{.}{2.3} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5} D{.}{.}{3.5}}
\toprule
 & \multicolumn{1}{c}{All Users} & \multicolumn{1}{c}{Low PM Share} & \multicolumn{1}{c}{High PM Share} & \multicolumn{1}{c}{Single-Home} & \multicolumn{1}{c}{Multi-Home} & \multicolumn{1}{c}{High UE MSA} & \multicolumn{1}{c}{High PM MSA} & \multicolumn{1}{c}{Low UE MSA} & \multicolumn{1}{c}{High UE + Single} & \multicolumn{1}{c}{High UE + Multi} & \multicolumn{1}{c}{High Share + Single} & \multicolumn{1}{c}{High Share + Multi} \\
\midrule
Intercept   & 0.00         & 0.00      & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         & 0.00         \\
            & (2.46)       & (2.18)    & (2.49)       & (1.82)       & (1.80)       & (2.04)       & (2.91)       & (2.56)       & (3.18)       & (1.66)       & (1.80)       & (2.16)       \\
Post-Merger & -40.68^{***} & -7.54^{*} & -50.00^{***} & -42.74^{***} & -27.85^{***} & -33.71^{***} & -38.61^{***} & -39.94^{***} & -62.01^{***} & -11.91^{***} & -43.63^{***} & -31.60^{***} \\
            & (3.53)       & (3.13)    & (3.57)       & (2.61)       & (2.59)       & (2.92)       & (4.18)       & (3.67)       & (4.57)       & (2.38)       & (2.58)       & (3.10)       \\
\midrule
R$^2$       & 0.80         & 0.15      & 0.86         & 0.89         & 0.78         & 0.80         & 0.72         & 0.78         & 0.85         & 0.43         & 0.90         & 0.76         \\
Adj. R$^2$  & 0.79         & 0.12      & 0.85         & 0.89         & 0.77         & 0.80         & 0.71         & 0.78         & 0.84         & 0.41         & 0.89         & 0.75         \\
Num. obs.   & 35           & 35        & 35           & 35           & 35           & 35           & 35           & 35           & 35           & 35           & 35           & 35           \\
\bottomrule
\multicolumn{13}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\caption{B\&P: Level Shift in Detrended Period FEs at Merger (Dec 2020)}
\label{tab:bp_break_tests}
\end{center}
\end{table}



==> tex/APC_table3_BP_all_DVs.tex <==

\begin{table}[htbp]
\begin{center}
\begin{tabular}{l D{.}{.}{3.5} D{.}{.}{2.5} D{.}{.}{2.5} D{.}{.}{2.5} D{.}{.}{2.5} D{.}{.}{3.5}}
\toprule
 & \multicolumn{1}{c}{\% Postmates} & \multicolumn{1}{c}{\% UberEats} & \multicolumn{1}{c}{\% DoorDash} & \multicolumn{1}{c}{\% GrubHub} & \multicolumn{1}{c}{Orders} & \multicolumn{1}{c}{Spend} \\
\midrule
Intercept   & 0.00         & -0.00       & -0.00       & -0.00      & 0.00        & 0.00         \\
            & (2.46)       & (1.45)      & (1.05)      & (0.47)     & (0.15)      & (5.52)       \\
Post-Merger & -40.68^{***} & 20.79^{***} & 15.38^{***} & 4.96^{***} & -1.04^{***} & -44.11^{***} \\
            & (3.53)       & (2.08)      & (1.51)      & (0.68)     & (0.22)      & (7.92)       \\
\midrule
R$^2$       & 0.80         & 0.75        & 0.76        & 0.62       & 0.41        & 0.48         \\
Adj. R$^2$  & 0.79         & 0.74        & 0.75        & 0.61       & 0.39        & 0.47         \\
Num. obs.   & 35           & 35          & 35          & 35         & 35          & 35           \\
\bottomrule
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\caption{B\&P: Post-Merger Level Shift in Detrended Period FEs by DV}
\label{tab:bp_break_dvs}
\end{center}
\end{table}



==> tex/APC_table5_spec_curve_controls.tex <==
\begin{table}[htbp]
\centering
\caption{B\&P Specification Curve: Post-Merger Break in Period FEs Across Control Sets}
\label{tab:bp_spec_curve}
\begin{tabular}{lcccc}
\hline\hline
Specification & Break (pp) & SE & p-value & 95\% CI \\
\hline
1: No controls & -26.999 & (2.736) & 0.0000 & [-32.361, -21.636] \\
2: + User (sync, multi) & NA & (NA) & NA & [NA, NA] \\
3: + COVID & -27.631 & (2.609) & 0.0000 & [-32.745, -22.517] \\
4: + Restaurants (full) & -27.631 & (2.609) & 0.0000 & [-32.745, -22.517] \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Controls added cumulatively. User $\times$ time: issyncing, multi-homing indicators.} \\
\multicolumn{5}{l}{\footnotesize COVID: standardized cases (+ squared), workplace closures, gathering restrictions, stay-at-home.} \\
\multicolumn{5}{l}{\footnotesize Restaurant supply: new/common restaurants on Postmates and other platforms.} \\
\end{tabular}
\end{table}


==> tex/empirical_methodology.tex <==
% ========================================================================
% EMPIRICAL METHODOLOGY AND RESULTS
% ========================================================================

\section{Empirical Strategy}\label{sec:empirical_strategy}

\subsection{Sample Construction}\label{subsec:sample}

Our analysis focuses on consumers who used Postmates prior to the merger announcement in December 2020. We construct the analysis sample through the following steps. First, we restrict to users with at least one Postmates transaction before December 2020 in a metropolitan statistical area (MSA) containing at least 10 such users. For users appearing in multiple MSAs, we assign them to their primary MSA based on the highest number of total orders. We then apply two data quality filters: (i) we remove users whose pre-merger Postmates budget share is below 5\%, as these represent negligible Postmates engagement; and (ii) we remove users who had zero Postmates spending in more than 50\% of their post-adoption pre-merger months, as these represent users who had effectively disengaged from the platform before the merger.

\subsection{Treatment Assignment}\label{subsec:treatment}

We exploit geographic variation in UberEats' pre-merger market presence to construct our treatment variable. For each MSA, we compute UberEats' pre-merger market share as the fraction of total food delivery spending (across UberEats, Postmates, DoorDash, and GrubHub) captured by UberEats:
\begin{equation}\label{eq:market_share}
    \text{UE\_Share}_{m} = \frac{\sum_{i \in m} \text{Spending}_{i,\text{UberEats},\text{pre}}}{\sum_{i \in m} \sum_{p \in \mathcal{P}} \text{Spending}_{i,p,\text{pre}}}
\end{equation}
where $m$ indexes MSAs, $i$ indexes consumers, $p$ indexes platforms, and $\mathcal{P} = \{\text{UberEats, Postmates, DoorDash, GrubHub}\}$ is the set of all platforms. The pre-merger period is defined as all months before December 2020.

MSAs are assigned to the treatment group if their UberEats market share exceeds the sample median:
\begin{equation}\label{eq:treatment}
    \text{Treated}_{m} = \mathbf{1}\left[\text{UE\_Share}_{m} > \text{Median}(\text{UE\_Share})\right]
\end{equation}

The intuition is that in MSAs where UberEats had a stronger pre-merger presence, the acquisition of Postmates would produce a larger competitive shock---effectively consolidating a greater share of the local market under a single firm. Consumers in high-UberEats-share MSAs are thus more ``treated'' by the merger.

% FIGURE: UberEats Market Share Across MSAs
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig3_ubereats_market_share.pdf}
    \caption{Pre-Merger UberEats Market Share by MSA. Treatment assigned to MSAs above the median UberEats market share (dashed red line).}
    \label{fig:ue_market_share}
\end{figure}

\subsection{Pre-Merger Postmates Budget Share Categories}\label{subsec:budget_share}

To examine heterogeneous effects by consumer dependence on Postmates, we categorize users based on their pre-merger Postmates spending share:
\begin{equation}\label{eq:budget_categories}
    \text{Category}_{i} = \begin{cases}
        \text{Low}    & \text{if } s_{i,\text{PM}} < 25\% \\
        \text{Medium} & \text{if } 25\% \leq s_{i,\text{PM}} \leq 70\% \\
        \text{High}   & \text{if } s_{i,\text{PM}} > 70\%
    \end{cases}
\end{equation}
where $s_{i,\text{PM}}$ is the share of consumer $i$'s total pre-merger food delivery spending allocated to Postmates. Consumers in the ``High'' category are those most dependent on Postmates and therefore most exposed to changes in Postmates' competitive position following the merger.

% FIGURE: Distribution of Pre-Merger Postmates Spending Share
\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/fig1_pm_share_distribution.pdf}
    \caption{Distribution of Pre-Merger Postmates Spending Share. Dashed lines indicate category cutoffs at 25\% and 70\%.}
    \label{fig:pm_share_dist}
\end{figure}

\subsection{Difference-in-Differences Specification}\label{subsec:did}

Our main estimating equation is a two-way fixed effects difference-in-differences model:
\begin{equation}\label{eq:did_main}
    y_{imt} = \alpha + \beta \cdot (\text{Treated}_{m} \times \text{Post}_{t}) + \mathbf{X}'_{imt}\boldsymbol{\gamma} + \mu_{m} + \lambda_{t} + \varepsilon_{imt}
\end{equation}
where $y_{imt}$ is the percentage of total food delivery spending allocated to Postmates by consumer $i$ in MSA $m$ at month $t$; $\text{Treated}_{m}$ is the binary treatment indicator defined in Equation~\eqref{eq:treatment}; $\text{Post}_{t} = \mathbf{1}[t \geq \text{Dec 2020}]$ indicates the post-merger period; $\mu_{m}$ and $\lambda_{t}$ are MSA and year-month fixed effects, respectively; and $\varepsilon_{imt}$ is the error term, clustered at the MSA level.

The coefficient $\beta$ captures the average treatment effect on the treated---the differential change in Postmates spending share for consumers in high-UberEats-share MSAs relative to those in low-UberEats-share MSAs, after the merger.

\begin{comment}

The vector $\mathbf{X}_{imt}$ includes the following control variables, added cumulatively across specifications:

\begin{enumerate}
    \item \textbf{Sync status} (\texttt{issyncing}): Whether the consumer's email receipt collection remains active
    \item \textbf{Postmates tenure}: Months from first Postmates order to the merger date
    \item \textbf{COVID controls}: Standardized total COVID cases and its square, workplace closure indicators (partial and full), gathering restrictions ($\leq$10 and $\leq$100 persons), and stay-at-home orders, all at the MSA-month level
    \item \textbf{Multi-platform indicators}: Binary variables for whether the consumer also used UberEats, DoorDash, or GrubHub before the merger
    \item \textbf{Budget share categories}: Indicators for Low ($<$25\%) and High ($>$70\%) pre-merger Postmates spending share
    \item \textbf{Restaurant controls}: Number of new and continuing (common) restaurants on Postmates and on other platforms, measured at the user-MSA level
\end{enumerate}
\end{comment}
\subsection{Heterogeneous Effects by Postmates Dependence}\label{subsec:het_effects}

To test whether the merger disproportionately affected consumers who were most dependent on Postmates, we estimate an augmented model with an interaction term:
\begin{equation}\label{eq:did_interaction}
    y_{imt} = \alpha + \beta_{1} \cdot \text{DiD}_{mt} + \beta_{2} \cdot \text{DiD}_{mt} \times \text{HighShare}_{i} + \delta_{1} \cdot \text{LowShare}_{i} + \delta_{2} \cdot \text{HighShare}_{i} + \mathbf{X}'_{imt}\boldsymbol{\gamma} + \mu_{m} + \lambda_{t} + \varepsilon_{imt}
\end{equation}
where $\text{DiD}_{mt} = \text{Treated}_{m} \times \text{Post}_{t}$, $\text{HighShare}_{i} = \mathbf{1}[s_{i,\text{PM}} > 70\%]$, and $\text{LowShare}_{i} = \mathbf{1}[s_{i,\text{PM}} < 25\%]$. The coefficient $\beta_{2}$ captures the \emph{additional} effect of the merger on high-Postmates-share consumers in treated MSAs relative to low/medium-share consumers.

\subsection{Event Study Specification}\label{subsec:event_study}

To examine the dynamic effects of the merger and validate the parallel trends assumption, we estimate an event study specification:
\begin{equation}\label{eq:event_study}
    y_{imt} = \alpha + \sum_{\substack{\tau = \underline{\tau} \\ \tau \neq -1}}^{\bar{\tau}} \beta_{\tau} \cdot \mathbf{1}[t - t^{*} = \tau] \times \text{Treated}_{m} + \mathbf{X}'_{imt}\boldsymbol{\gamma} + \mu_{m} + \lambda_{\tau} + \varepsilon_{imt}
\end{equation}
where $\tau = t - t^{*}$ denotes months relative to the merger date ($t^{*} = \text{Dec 2020}$), and $\tau = -1$ (November 2020) serves as the reference period. Pre-merger coefficients $\{\beta_{\tau}\}_{\tau < 0}$ test the parallel trends assumption: if the identifying assumption holds, these coefficients should be statistically indistinguishable from zero.

We estimate this for both the full sample and the high-Postmates-share subgroup ($s_{i,\text{PM}} > 70\%$), with and without the full set of controls described above.


\section{Descriptive Statistics}\label{sec:descriptives}

% TABLE 2: Summary Statistics
\input{tabs/table2_summary_statistics.tex}

% TABLE 3: Balance Table
\input{tabs/table3_balance_table.tex}

% TABLE 4: Spending Share Categories
\input{tabs/table4_share_categories.tex}

% TABLE 5: MSA-Level Summary
\input{tabs/table5_msa_summary.tex}

% FIGURE: Parallel Trends
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig2_parallel_trends.pdf}
    \caption{Mean Percentage of Spending on Postmates Over Time, by Treatment Group. Treatment group consists of MSAs with above-median pre-merger UberEats market share. Shaded bands indicate 95\% confidence intervals.}
    \label{fig:parallel_trends}
\end{figure}

% FIGURE: Platform Composition Over Time
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig4_platform_composition.pdf}
    \caption{Average Platform Spending Shares Over Time Among Pre-Merger Postmates Users.}
    \label{fig:platform_composition}
\end{figure}

% FIGURE: Multi-Platform Usage
\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{figs/fig5_multi_platform.pdf}
    \caption{Multi-Platform Usage Among Postmates Users Before the Merger.}
    \label{fig:multi_platform}
\end{figure}

% FIGURE: Postmates Tenure Distribution
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/fig6_tenure_distribution.pdf}
    \caption{Distribution of Postmates Tenure (Months from First Order to Merger).}
    \label{fig:tenure}
\end{figure}

% FIGURE: Users Per Month
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig7_users_per_month.pdf}
    \caption{Number of Active Users Per Month by Treatment Group.}
    \label{fig:users_per_month}
\end{figure}

% FIGURE: Balance Plot
\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/fig8_balance_plot.pdf}
    \caption{Standardized Mean Differences Between Treatment and Control Groups. Dashed lines indicate the $\pm 0.1$ balance threshold.}
    \label{fig:balance_plot}
\end{figure}

% FIGURE: Trends by Spending Share Category
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig9_trends_by_share.pdf}
    \caption{Mean Postmates Spending Share Over Time by Budget Share Category and Treatment Group.}
    \label{fig:trends_by_share}
\end{figure}


\section{Results}\label{sec:results_methodology}

\subsection{Main DiD Results: Specification Curve}\label{subsec:spec_curve}

We present results from a specification curve analysis that progressively adds control variables to the baseline two-way fixed effects model. This approach demonstrates the stability of our estimates across different modeling choices.

% FIGURE: Specification Curve - DiD
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/spec_curve_did_simple.pdf}
    \caption{Specification Curve: DiD Coefficient on Percentage Postmates Spending. Each specification cumulatively adds controls. Error bars indicate 95\% confidence intervals with standard errors clustered at the MSA level.}
    \label{fig:spec_curve_did}
\end{figure}

The specification curve in Figure~\ref{fig:spec_curve_did} plots the DiD coefficient $\hat{\beta}$ from Equation~\eqref{eq:did_main} across eight specifications that progressively add controls: (1)~MSA and time fixed effects only; (2)~sync status; (3)~Postmates tenure; (4)~COVID-19 controls; (5)~multi-platform indicators; (6)~budget share categories; (7)~Postmates restaurant controls; and (8)~the full model including other-platform restaurant controls.

\subsection{Heterogeneous Effects: High Postmates Share Interaction}\label{subsec:het_results}

% FIGURE: Specification Curve - DiD x High Share
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/spec_curve_did_high_share.pdf}
    \caption{Specification Curve: DiD $\times$ High Share Coefficient. The coefficient on the interaction between the DiD term and an indicator for consumers with $>$70\% pre-merger Postmates spending share.}
    \label{fig:spec_curve_high_share}
\end{figure}

Figure~\ref{fig:spec_curve_high_share} presents the specification curve for the interaction coefficient $\hat{\beta}_{2}$ from Equation~\eqref{eq:did_interaction}, capturing the differential effect on high-dependence Postmates consumers.

\subsection{Event Study Results}\label{subsec:event_results}

% FIGURE: Event Study - All Users
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/event_study_did_comparison.png}
    \caption{Event Study: Effect on Percentage Postmates Spending (All Users). Coefficients from Equation~\eqref{eq:event_study} with and without controls. Reference period is month $-1$ (November 2020).}
    \label{fig:event_study_all}
\end{figure}

% FIGURE: Event Study - High Share Users
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/event_study_high_share_comparison.png}
    \caption{Event Study: High Postmates Share Subgroup ($>$70\% Pre-Merger Spending Share). Reference period is month $-1$ (November 2020).}
    \label{fig:event_study_high}
\end{figure}

% FIGURE: Event Study - Combined
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/event_study_combined.png}
    \caption{Event Study: All Users vs.\ High Share Subgroup (Full Controls). Comparison of dynamic treatment effects for the full sample and the high-dependence subgroup.}
    \label{fig:event_study_combined}
\end{figure}

Figures~\ref{fig:event_study_all}--\ref{fig:event_study_combined} present the event study estimates. Pre-merger coefficients that are close to zero and statistically insignificant would support the parallel trends assumption underlying our identification strategy.


\section{Robustness Checks}\label{sec:robustness}

\subsection{Sensitivity to Sample Restrictions}\label{subsec:robust_filters}

Our baseline sample applies two filters: (i)~removing users with less than 5\% pre-merger Postmates budget share, and (ii)~removing users with zero Postmates spending in more than 50\% of their post-adoption pre-merger months. To ensure our results are not driven by these specific cutoffs, we re-estimate both the simple DiD and the DiD~$\times$~High Share models across a grid of alternative thresholds:
\begin{itemize}
    \item Zero-months threshold $x \in \{30\%, 40\%, 50\%, 60\%, 70\%, 80\%\}$: Users are removed if more than $x\%$ of their post-adoption pre-merger months have zero Postmates spending.
    \item Budget share threshold $y \in \{0\%, 2\%, 5\%, 10\%, 15\%\}$: Users are removed if their pre-merger Postmates budget share is below $y\%$.
\end{itemize}

% FIGURE: Robustness - DiD across filter thresholds
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/robust_did_coefficient.pdf}
    \caption{Robustness: DiD Coefficient Across Sample Restrictions. Each point represents the full-model DiD estimate under a different combination of zero-months ($x$) and budget share ($y$) filter thresholds. Error bars indicate 95\% CIs.}
    \label{fig:robust_did}
\end{figure}

% FIGURE: Robustness - DiD x High Share across filter thresholds
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/robust_did_high_share_coefficient.pdf}
    \caption{Robustness: DiD $\times$ High Share Coefficient Across Sample Restrictions.}
    \label{fig:robust_high_share}
\end{figure}

\subsection{Sensitivity to Exclusion Window}\label{subsec:robust_window}

As a further robustness check, we vary the exclusion window around the merger date. The baseline specification uses no exclusion window (post-period begins immediately in December 2020). We test alternative windows by varying the start date $\in \{\text{Oct 2020, Nov 2020, Dec 2020, Jan 2021}\}$ and end date $\in \{\text{Dec 2020, Jan 2021, Feb 2021, Mar 2021, Apr 2021}\}$, dropping all observations within the excluded interval. Treatment assignment is held fixed using the standard pre-December-2020 definition to avoid endogenous treatment reclassification.

% FIGURE: Robustness - Exclusion Window DiD
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/robust_exclusion_window_did.pdf}
    \caption{Robustness: DiD Coefficient Across Exclusion Windows. Labels indicate the number of excluded months. Treatment assignment is fixed at the pre-December-2020 definition.}
    \label{fig:robust_window_did}
\end{figure}

% FIGURE: Robustness - Exclusion Window DiD x High Share
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/robust_exclusion_window_did_high_share.pdf}
    \caption{Robustness: DiD $\times$ High Share Coefficient Across Exclusion Windows.}
    \label{fig:robust_window_high}
\end{figure}


==> tex/multihoming_avgcharged.tex <==
     33.59

==> tex/multihoming_avgcharged_postacq.tex <==
     34.65

==> tex/multihoming_avgcharged_preacq.tex <==
     32.51

==> tex/multihoming_avgnorders.tex <==
        50

==> tex/multihoming_avgnorders_postacq.tex <==
        42

==> tex/multihoming_avgnorders_preacq.tex <==
        33

==> tex/multihoming_median_norders.tex <==
        18

==> tex/multihoming_median_norders_postacq.tex <==
        18

==> tex/multihoming_median_norders_preacq.tex <==
        14

==> tex/multihoming_norder_perct.tex <==
     72.11

==> tex/multihoming_norder_perct_postacq.tex <==
     59.64

==> tex/multihoming_norder_perct_preacq.tex <==
     66.25

==> tex/multihoming_norders.tex <==
      192241

==> tex/multihoming_norders_postacq.tex <==
       84570

==> tex/multihoming_norders_preacq.tex <==
       82667

==> tex/multihoming_nusers.tex <==
3816

==> tex/multihoming_nusers_postacq.tex <==
2010

==> tex/multihoming_nusers_preacq.tex <==
2527

==> tex/multihoming_perct_users.tex <==
37.80

==> tex/multihoming_perct_users_postacq.tex <==
32.58

==> tex/multihoming_perct_users_preacq.tex <==
34.36

==> tex/multihoming_revenue.tex <==
     6457073

==> tex/multihoming_revenue_postacq.tex <==
     2930587

==> tex/multihoming_revenue_preacq.tex <==
     2687407

==> tex/multihoming_revperct.tex <==
     73.24

==> tex/multihoming_revperct_postacq.tex <==
     60.73

==> tex/multihoming_revperct_preacq.tex <==
     67.34

==> tex/nof_exitusers_postacq.tex <==
3924

==> tex/nof_newusers_postacq.tex <==
2739

==> tex/nofusers_preacq.tex <==
7355

==> tex/receipt_nreceipts.tex <==
266584

==> tex/receipt_nusers.tex <==
10094

==> tex/singlehoming_avgcharged.tex <==
     31.74

==> tex/singlehoming_avgcharged_postacq.tex <==
     33.12

==> tex/singlehoming_avgcharged_preacq.tex <==
     30.95

==> tex/singlehoming_avgnorders.tex <==
        12

==> tex/singlehoming_avgnorders_postacq.tex <==
        14

==> tex/singlehoming_avgnorders_preacq.tex <==
         9

==> tex/singlehoming_median_norders.tex <==
         2

==> tex/singlehoming_median_norders_postacq.tex <==
         3

==> tex/singlehoming_median_norders_preacq.tex <==
         2
